ScreenAvoider: Protecting Computer Screens from Ubiquitous Cameras

We live and work in environments that are inundated with cameras embedded in devices such as phones, tablets, laptops, and monitors. Newer wearable devices like Google Glass, Narrative Clip, and Autographer offer the ability to quietly log our lives with cameras from a `first person' perspective. While capturing several meaningful and interesting moments, a significant number of images captured by these wearable cameras can contain computer screens. Given the potentially sensitive information that is visible on our displays, there is a need to guard computer screens from undesired photography. People need protection against photography of their screens, whether by other people's cameras or their own cameras. We present ScreenAvoider, a framework that controls the collection and disclosure of images with computer screens and their sensitive content. ScreenAvoider can detect images with computer screens with high accuracy and can even go so far as to discriminate amongst screen content. We also introduce a ScreenTag system that aids in the identification of screen content, flagging images with highly sensitive content such as messaging applications or email webpages. We evaluate our concept on realistic lifelogging datasets, showing that ScreenAvoider provides a practical and useful solution that can help users manage their privacy.

==> ack.tex <==
% !TEX root = main.tex

\section*{Acknowledgment}

This material is based upon work supported by the National Science
Foundation under grants XX. This
work was also partially funded by the Office of the Vice Provost of
Research at Indiana University Bloomington through the Faculty
Research Support Program.  We thank the anonymous reviewers for their
valuable comments and John McCurley for his editorial help.

